LoRID: Low-Rank Iterative Diffusion for Adversarial Purification

This work presents an information-theoretic examination of diffusion-based purification methods, the state-of-the-art adversarial defenses that utilize diffusion models to remove malicious perturbations in adversarial examples. By theoretically characterizing the inherent purification errors associated with the Markov-based diffusion purifications, we introduce LoRID, a novel Low-Rank Iterative Diffusion purification method designed to remove adversarial perturbation with low intrinsic purification errors. LoRID centers around a multi-stage purification process that leverages multiple rounds of diffusion-denoising loops at the early time-steps of the diffusion models, and the integration of Tucker decomposition, an extension of matrix factorization, to remove adversarial noise at high-noise regimes. Consequently, LoRID increases the effective diffusion time-steps and overcomes strong adversarial attacks, achieving superior robustness performance in CIFAR-10/100, CelebA-HQ, and ImageNet datasets under both white-box and black-box settings.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
Despite being widely used, neural networks are incredibly vulnerable to minuscule perturbations in the input space, perturbations purposely constructed to cause unpredictable outputs, often leading to undesired or fatal behavior. This type of perturbation is commonly dubbed as an \textit{adversarial attack}~\cite{szegedy2014intriguing}~\cite{goodfellow2015explaining}, and over the last few years, there have been numerous strategies derived in an attempt to protect vulnerable models~\cite{app9050909}.
\textit{Adversarial training}, that is training the vulnerable model directly with possible adversarial attacks derived from the training distribution, seems to be a temporary solution at the moment~\cite{madry2019deep}\cite{bai2021recent}\cite{zhang2019theoretically}, as often times models are limited by their bandwidth and can only defend  well against specific attacks that were used during adversarial training due to the increase in complexity~\cite{wong2020fast}. Current research also suggests that adversarial training might not be a viable solution for obtaining models with desirable robustness and accuracy; with a large intrinsic limitation of adversarial training being the trade-off
between robustness and generalization~\cite{zhang2019theoretically}.
\\\\
\textit{adversarial purification} is another common technique used to defend against adversarial attacks. \textit{Adversarial purification} techniques rely on generative models, dubbed purifiers, trained to restore the adversarial image towards the most likely pre-attacked image~\cite{salakhutdinov2015learning}\cite{shi2021online}\cite{song2018pixeldefend}.  The main benefit of utilizing \textit{adversarial purification} is the inherent decoupled nature of the purifiers themselves, as typically the purifier is trained independently of a classifier. This allows for a purifier to be utilized for any external model without the need for retraining/reconfiguration of any sort required by the external model. However, in practice, it is an ongoing area of research in constructing a generative model that is able to achieve far greater performance then adversarial training techniques~\cite{croce2020reliable}; possibly due to problems such as: the ambiguity of necessary semantic content needed from the attacked image for the classification model to predict the correct output~\cite{10.1007/978-3-030-84522-3_37}, Mode collapse~\cite{goodfellow2014generative}, and attacks that generate extreme out-of-distribution observations ~\cite{zhang2021understanding}.
\\\\
Diffusion models have recently gained interest and currently serve as a fairly population class of generative model, due to their performance in generating high sample quality from isotopic Gaussian samples~\cite{ho2020denoising}\cite{rombach2022highresolution}\cite{song2021scorebased}. What perhaps sets a diffusion model apart from other generative models is their inherit stochastic generation of samples, which serves as a strong basis as it has been seen (in the field of online learning) the strength of stochastic decision making when facing a possible stream of adversarial samples~\cite{rakhlin2011online}. Due to this trait, diffusion models serve as a natural extension towards being utilized as a purifier~\cite{nie2022diffusion}\cite{wang2022guided}, given the deniosing property that allows for generation of samples typically influenced by the training distribution. 
\\\\
\Geigh{To make the smooth transistion, Start the context speaking about low rank approximation, particularly for adversarial defense. Cite papers that exploit low rank approximation for adversarial robustness (borrow from adversarialtensors paper related work section), describe their strengths,flaws and thier sub-par performance. Bring our previous adversarialtensor paper in context and mention that how a simple low rank approximation is able to achieve significant performance compared to state of the art but has its own deficienceies.The story should be can be combine such abilities of low rank approximation with complex denosing diffusion models}
The \textit{Tucker decomposition}, a higher-order extension of matrix factorization, has demonstrated its efficacy in extracting latent features from multi-dimensional data~\cite{rabanser2017introduction}. By decomposing an image into a core tensor and factor matrices along each mode, Tucker decomposition excels in capturing both local and global dependencies within the data. This unique capability positions it as a promising alternative to traditional learned latent inputs~\cite{gillet:hal-03892165}. 
\\\\

%In this paper, we delve into the rationale behind leveraging Tucker decomposition as the latent input for latent diffusion purification. We argue that this approach not only reduces the model complexity of latent space diffusion models but also fosters improved, model agnostic generalization across datasets. By incorporating the inherent structure present in Tucker decomposition, we aim to demonstrate its potential in facilitating a robust and efficient purification of observations compared to conventional learned latent inputs. 

In this study, we explore the utility of the Tucker decomposition for deriving a low-rank projection basis from datasets, aimed at achieving a compressed representation that serves as the latent input for denoising diffusion processes. Our approach leverages the reduced complexity afforded by operating in latent space, potentially enhancing model generalization across diverse datasets in a model-agnostic manner. By capitalizing on the structured compression of Tucker decomposition, we demonstrate its efficacy in enabling robust and efficient purification of data, surpassing traditional methods that rely on learned latent inputs.

\paragraph{In summary, our contributions are:}
\begin{itemize}
    \item We propose the first low rank latent denoising diffusion model  based adversarial purification framework, that proposes a trainable free decoder and encoder.
    \item Our multi-stage denoising strategy harnesses the synergistic potential of low-rank approximation and diffusion models, targeting both coarse and fine-grained noise levels, to efficiently counteract adversarial perturbations across a broad spectral spectrum.
    \item We provide \Geigh{we would like to show how tucker decomposition fits in all this}.
    \item We provide \Geigh{Need to add anaylsis towards insight for stopping time for the denoising}
\end{itemize}



==> sec/2_background.tex <==
\section{Background}
\label{sec:Background}
\paragraph{Tucker Decomposition} also known as higher-order singular value decomposition (HOSVD)~\cite{5447070}, is a mathematical technique used in multilinear algebra and data analysis, and can be viewed as an extension of the concept of singular value decomposition (SVD) for higher-dimensional data arrays or tensors~\cite{doi:10.1137/07070111X}. Computing the Tucker decomposition for some given tensor $\mathcal{X}$, results in finding a representation of $\mathcal{X}$ as a core tensor multiplied by a set of factor matrices along each mode (dimension). The core tensor contains the core information of the original tensor, while the factor matrices capture the relationships between the modes. Formally, for a tensor $\mathcal{X}$ of size $I_1 \times I_2 \times ... \times I_N$, the Tucker decomposition can be written as: \begin{equation*}
    \mathcal{X} =\mathcal{G} \times_1 U_1 \times_2 U_2 \times_3 ... \times_N U_N
\end{equation*}
 Where:
 \begin{itemize}
     \item  $\mathcal{G}$ is the core tensor of size $r_1 \times r_2 \times ... \times r_N$ for $r_n \leq I_n$ where $n = 1,2, ..,N$.
     \item $U_n$ is the factor matrix for mode $n$ with size $I_n \times r_n$, where each column represents the basis vector along mode $n$.
     \item $\times_n$ denotes the mode-$n$ product, which is a contraction along mode $n$ between a tensor and a matrix.
 \end{itemize}
 Computing the tucker decomposition can allow for dimension reduction through capture of the essential structure of the tensor in terms of its core tensor and factor matrices. It's widely used in various fields such as signal processing, image processing, neuroscience, data compression, and in the line of the proposed work, feature extraction from high-dimensional data~\cite{kolda2009tensor}.

 

\paragraph{Denoising Diffusion Probabilistic Model (DDPM)}
DDPMs are a class of generative models that work by iteratively adding noise to an input signal (forward process), then learning to "denoise" from a noisy signal to generate new samples, similar to the ones previously seen in the training distribution~\cite{ho2020denoising}. 
\paragraph{Forward diffusion process}
Formally, given a data point sampled from a real data distribution $x_0 \sim q(x)$, a \textit{forward diffusion process} is a process of which small amounts of Gaussian noise are applied to $x_0$, producing a sequence of noisy samples $x_1,. . ., x_T$. Step sizes are controlled by a variance schedule $\{\beta_t\in (0,1)\}^T_{t=1}$, where the schedule is typically chosen in a conventional fashion to aid in sample quality~\cite{chen2023importance}. Single Markovian steps between sequential $x's$ are defined as:
\begin{equation}
\label{eq:single_step_forward}
   q(x_{t}|x_{t-1}) := \mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1},\beta_t I) 
\end{equation}
where the total trajectory can be computed as:
\begin{equation}
    q(x_{1:T}|x_0) = \Pi^{T}_{t=1}q(x_t|x_{t-1})
\end{equation}
The data sample $x_0$ is expected to gradually loose features that resemble the original distribution, as the step $t$ becomes larger and eventually become equivalent to an isotropic Gaussian distribution.
\paragraph{Backward diffusion process}
Typically a U-Net is trained to reverse the forward process, and sample from $q(x_{t-1}|x_t)$, 
\Geigh{TODO Backward Process in latex}
\paragraph{Purification }


==> sec/3_approach.tex <==
\section{Approach}
\label{sec:Approach}
\subsection{Factors as a basis for a projected space}
Transforming data into a latent space before can add a layer of obfuscation against adversarial attacks. Adversarial perturbations designed to fool models in the original image space may not translate as effectively into the latent space. However, a latent space needs to be able to be reasonably constructed such that significant features are preserved~\cite{asperti2023comparing}.
To satisfy this constraint but also eliminate the necessity of deriving a learnable decoder and encoder~\cite{rombach2022highresolution}, we instantiate a static projection based on the tucker decomposition of the original dataset that allows us to directly compute a latent projection of an observation $x$ i.e $x \mapsto x^{\prime}$, effectively reducing the model complexity, increases the ease of regularization, and allows us to project into a well studied subspace~\cite{rabanser2017introduction}. Theorem~\ref{thr:tucker_error_compression_bound} confirms that utilization of the Tucker decomposition can indeed derive a sufficient latent space for $x_0$ to be projected onto, with some level of desired expected compression.
\begin{theorem}
\label{thr:tucker_error_compression_bound}
Given a tensor $\mathcal{X}$ of dimensions $ I_1 \times I_2 \times \cdots \times I_N $, and its Tucker decomposition resulting in a core tensor $\mathcal{G}$ of dimensions $r_1 \times r_2 \times \cdots \times r_N $, and factor matrices $U^{(n)}$ of size $I_n \times r_n $ for each mode $ n $, with the compression ratio $C$~\cite{doi:10.1137/07070111X} defined as
\begin{align}
    C = \frac{\prod_{n=1}^{N} I_n}{\prod_{n=1}^{N} r_n + \sum_{n=1}^{N} I_n r_n}, 
\end{align}
and assuming the omitted singular values (or their tensor equivalents) follow a predictable decay pattern allowing for an average squared singular value $ \overline{\sigma^2} $ for omitted components, the reconstruction error $E$, measured by the Frobenius norm $||\mathcal{X} - \hat{\mathcal{X}}||_F$ where $\hat{\mathcal{X}}$ is the tensor reconstructed from $\mathcal{G} $ and $ U^{(n)} $, can be approximated by an error bound $\epsilon$ that is influenced by the choice of ranks $ \{r_n\} $ and the inherent data structure captured in the omitted singular values:
\begin{align}
\epsilon \approx \sum_{n=1}^{N} \sum_{i=r_n+1}^{I_n} (\sigma_{i_n}^{(n)})^2. 
\end{align}
Simplifying under the assumption of a uniform decay rate of singular values across modes, and denoting \( \overline{\sigma^2} \) as the average of squared omitted singular values, the bound can be further approximated as:
\begin{align}
\epsilon \propto \sum_{n=1}^{N} (I_n - r_n) \cdot \overline{\sigma^2}. 
\end{align}
Furthermore, considering the relationship between the reconstruction error bound \( \epsilon \) and the compression ratio \( C \) can be described by the function $f(C)$, where $\epsilon = f(C)$
is inversely related to $ C $. Specifically, as $ C$ increases (indicating higher compression),$\epsilon$ also increases, reflecting a higher loss of information due to the reduction in dimensions. Conversely, as $C$ decreases (lower compression, more information retained), $\epsilon$ decreases, indicating a lower reconstruction error. The specific form of $f(C)$ depends on the distribution and decay rate of the singular values associated with $\mathcal{X}$.
\end{theorem}
Given the chosen subspace, we adjust previous theoretical justifications regrading diffusion based purification discussed in~\cite{song2021maximum}\cite{lyu2012interpretation}\cite{wang2022guided}\cite{nie2022diffusion} to take in consideration the resulting subspace.
%\Geigh{Have not checked Theorem 3.3, 3.4 or main approach yet. Expect lots to be moved around.}



\subsection{Diffusion Purification on Low-Rank Projections} 

Denoising Diffusion Probabilistic Models (DDPMs)~\cite{ho2020denoising} are a class of generative models that work by iteratively adding noise to an input signal (the forward process), then learning to "denoise" from a noisy signal to generate new samples (the reverse process). Given a data point $\bmx_0$ sampled from the data distribution $ q(\bmx_0)$, a \textit{forward diffusion process} is a a Markov chain that gradually adds Gaussian noise to the data according to a variance schedule $\{\beta_t\in (0,1)\}^T_{t=1}$:
\begin{align}
    q( \bmx_{1:T}|\bmx_0) &:= \prod^{T}_{t=1}q(\bmx_t|\bmx_{t-1}) \\
   q(\bmx_{t}|\bmx_{t-1}) &:= \mathcal{N}(\bmx_t;\sqrt{1-\beta_t}\bmx_{t-1},\beta_t \mathbf{I}) \label{eq:forward}
\end{align}
The joint distribution $p_{\theta}(\bmx_{0:T})$ is called the reverse process, and it is defined as a Markov chain with learned Gaussian transitions starting at $p(\bmx_T) = \mathcal{N}(\bmx_T; \mathbf{0}, \mathbf{I})$:
\begin{align}
p_{\theta}(\bmx_{0:T}) &:= p(\bmx_T) \prod_{t=1}^{T} p_{\theta}(\bmx_{t-1} | \bmx_t), \\
p_{\theta}(\bmx_{t-1} | \bmx_t) &:= \mathcal{N}(\bmx_{t-1}; \boldsymbol{\mu}_{\theta}(\bmx_t, t), \mathbf{\Sigma}_{\theta}(\bmx_t, t))
\end{align}
A notable property of the forward process is that it admits sampling $\bmx_t$ at an arbitrary timestep $t$ in closed form: using the notation $\alpha_t := 1 - \beta_t$ and $\bar{\alpha}_t := \prod_{s=1}^{t} \alpha_s$, we have
\[
q(\bmx_t | \bmx_0) = \mathcal{N}\left(\bmx_t; \bar{\alpha}_t \bmx_0, (1 - \bar{\alpha}_t) \mathbf{I}\right)
\]

\subsubsection*{Convergence of KL divergence in DDPM} \label{sect:note1}
The work~\cite{nie2022DiffPure} previously considered a continuous version of the DDPMs and showed that two data distributions $q^{(1)}(\bmx_0)=q^{(1)}_{t=0}$ and $q^{(2)}(\bmx_0)=q^{(2)}_{t=0}$ get closer over the forward diffusion process, i.e., $ \nicefrac{\partial D_{KL}\left(q^{(1)}_t || q^{(2)}_t \right)}{\partial t} \leq 0 $. In the following, we establish the counterpart for the DDPM in the following theorem. 

\begin{theorem} \label{theorem:ddpm_converge}
Let $\left\{\bmx^{(i)}_t \right\}_{t \in \{0,...,T \}}$ be two diffusion processes defined by the forward Eq. (\ref{eq:forward}) for $i \in \{1,2\}$. We denote by $q^{(i)}_t$ the respective distributions of $\bmx_t^{(i)}$, i.e., $\bmx_t^{(1)} \sim q^{(1)}_{t}$ and $\bmx_t^{(2)}\sim q^{(2)}_{t}$. We then have
\begin{align*}
    D_{KL}\left(q^{(1)}_t||q^{(2)}_t \right) \geq D_{KL}\left(q^{(1)}_{t+1}||q^{(2)}_{t+1} \right), \quad \forall t = 0,\cdots, T-1.
\end{align*}
\end{theorem}
\begin{proof}
We start by restating the \textit{chain rule for relative entropy}~\cite{Cover2006}:
\begin{align}
    D_{KL}\left(p(\bmz_1,\bmz_2)||p'(\bmz_1,\bmz_2) \right)& = D_{KL}\left(p(\bmz_1)||p'(\bmz_1) \right) + \nonumber\\
    &D_{KL}\left(p(\bmz_2| \bmz_1)||p'(\bmz_2 | \bmz_1) \right)
\end{align}
Then, by denoting $q^{(i)}(\bmx_{t+1}, \bmx_t)$ the joint distribution of $\bmx^{(i)}_{t+1}$ and $ \bmx^{(i)}_t$, the chain rule gives us:
\begin{align}
     &D_{KL}\left( q^{(1)}(\bmx_{t+1}, \bmx_t) ||q^{(2)}(\bmx_{t+1}, \bmx_t) \right)  \\
     = \ & D_{KL}\left( q^{(1)}_{t+1} ||q^{(2)}_{t+1} \right) + D_{KL}\left( q^{(1)}(\bmx_{t}| \bmx_{t+1}) ||q^{(2)}(\bmx_{t} | \bmx_{t+1}) \right) \\
     = \ & D_{KL}\left( q^{(1)}_{t} ||q^{(2)}_{t} \right) + D_{KL}\left( q^{(1)}(\bmx_{t+1}| \bmx_{t}) ||q^{(2)}(\bmx_{t+1} | \bmx_{t}) \right) \label{eq:KLchainrule}
\end{align}
Note that, due to Eq. (\ref{eq:forward}), we have $ q^{(1)}(\bmx_{t+1}| \bmx_{t}) = q^{(2)}(\bmx_{t+1} | \bmx_{t})$, this implies the last term of Eq. (\ref{eq:KLchainrule}) $D_{KL}\left( q^{(1)}(\bmx_{t+1}| \bmx_{t}) ||q^{(2)}(\bmx_{t+1} | \bmx_{t}) \right) =0 $. Thus, we have:
\begin{align}
    D_{KL}\left( q^{(1)}_{t+1} ||q^{(2)}_{t+1} \right) +& D_{KL}\left( q^{(1)}(\bmx_{t}| \bmx_{t+1}) ||q^{(2)}(\bmx_{t} | \bmx_{t+1}) \right) \nonumber \\
     &=  D_{KL}\left( q^{(1)}_{t} ||q^{(2)}_{t} \right) 
\end{align}
Due to the nonnegativity of $D_{KL}\left( q^{(1)}(\bmx_{t}| \bmx_{t+1}) ||q^{(2)}(\bmx_{t} | \bmx_{t+1}) \right) $, we have the Theorem:
\begin{align}
    D_{KL}\left(q^{(1)}_t||q^{(2)}_t \right) \geq D_{KL}\left(q^{(1)}_{t+1}||q^{(2)}_{t+1} \right).
\end{align}
\end{proof}
\textbf{Remark.} The proof of Theorem~\ref{theorem:ddpm_converge} only relies on the fact that $ q^{(1)}(\bmx_{t+1}| \bmx_{t}) = q^{(2)}(\bmx_{t+1} | \bmx_{t})$, but not on the explicit form of that transition probability. Thus, it still holds for other adding-noise strategies.

\subsubsection*{Choosing the diffusion timestep for purification}

Intuitively, the diffusion timestep $t$ should be large enough to remove adversarial perturbations; however, a too-large $t$ will also remove the input's semantics. While the work~\cite{nie2022DiffPure} characterized how the diffusion timestep affects the difference between the clean image and purified image for continuous-time diffusion, we introduce the corresponding result for DDPM in the followings.


Using the reparameterize trick on the forward diffusion process, we have
\begin{align}
    \bmx_t = \sqrt{\bar{\alpha}_t} \bmx_0 + \sqrt{1 - \bar{\alpha}_t}\boldsymbol{\epsilon}_0
\end{align}
For the reverse process, the recovered signal in DDPM is given by~\cite{ho2020denoising}:
\begin{align}
    \hat{\bmx}_0 = \frac{1}{\sqrt{\bar{\alpha}_t}} \bmx_t - \frac{\sqrt{1 - \bar{\alpha}_t}}{ \sqrt{\bar{\alpha}_t}}\boldsymbol{\epsilon}_{\theta}(\bmx_t)
\end{align}
where $\boldsymbol{\epsilon}_{\theta}$ is a function approximator trained by the DDPM to predict $\boldsymbol{\epsilon}$ from $\bmx_t$. Given that, we have
\begin{align}
    \hat{\bmx}_0 - \bmx_0 =  \frac{\sqrt{1 - \bar{\alpha}_t}}{ \sqrt{\bar{\alpha}_t}} \left( \boldsymbol{\epsilon}_0 - \boldsymbol{\epsilon}_{\theta}\left( \sqrt{\bar{\alpha}_t} \bmx_0 + \sqrt{1 - \bar{\alpha}_t}\boldsymbol{\epsilon}_0
    \right)\right)
\end{align}

In the training of the DDPM, we aim to maximize the ELBO:
\begin{align*}
&\mathbb{E}_{q(\bmx_1|\bmx_0)}\left[\log p_{\theta}(\bmx_0|\bmx_1)\right] 
 - D_{KL} \left(q(\bmx_T |\bmx_0) \| p(\bmx_T)\right)  - \nonumber \\
 &\sum_{t=2}^{T} \mathbb{E}_{q(\bmx_t|\bmx_0)}\left[D_{KL}\left(q(\bmx_{t-1}|\bmx_t, \bmx_0) \| p_{\theta}(\bmx_{t-1}|\bmx_t)\right)\right]
\end{align*}
In this expression, most of the optimization cost lies in the summation term, which dominates the first reconstruction term. From the forwarding diffusion, we know that:
\begin{align*}
    q(\bmx_{t-1}|\bmx_t, \bmx_0) = \mathcal{N}\left(\bmx_{t-1}; \boldsymbol{\mu}_q(\bmx_t, \bmx_0) ,\mathbf{\Sigma}_q(t) \right)
\end{align*}
where
\begin{align*}
    \boldsymbol{\mu}_q(\bmx_t, \bmx_0)  &= \frac{\sqrt{\alpha_t}(1 - \bar{\alpha}_{t-1})}{1 - \bar{\alpha}_{t}}\bmx_{t} + \frac{\sqrt{\bar{\alpha}_{t-1}}(1 - \alpha_{t})}{1 - \bar{\alpha}_{t}}\bmx_{0} \\
    \mathbf{\Sigma}_q(t) &=  \frac{(1 - \alpha_{t})(1 - \bar{\alpha}_{t-1})}{1 - \bar{\alpha}_{t}} \mathbf{I}
\end{align*}
In order to match the denoising transition step $p_\theta(\bmx_{t-1}|\bmx_t)$ to ground-truth denoising transition step $q(\bmx_{t-1}|\bmx_t, \bmx_0)$, we need to parameterize its mean $\boldsymbol{\mu}_\theta(\bmx_t, t) $
 as $p_\theta$ is not conditioned on $\bmx_0$. Thus, in DDPM,  $\boldsymbol{\mu}_\theta(\bmx_t, t) $ takes the following form:
 \begin{align}
      \boldsymbol{\mu}_\theta(\bmx_t, t) =  \frac{\sqrt{\alpha_t}(1 - \bar{\alpha}_{t-1})}{1 - \bar{\alpha}_{t}}\bmx_{t} + \frac{\sqrt{\bar{\alpha}_{t-1}}(1 - \alpha_{t})}{1 - \bar{\alpha}_{t}} \hat{\bmx}_\theta(\bmx_t, t)
 \end{align}
 
 
 the maximization of the ELBO is equivalent to finding $\theta$ that minimizes 

Denote $\bmx_{\theta}(\bmx_t, t)$ the reverse output of the DDPM given the state $\bmx_t$ and the reverse transition $p_\theta$.

\begin{align}
    \|\hat{\bmx} - \bmx_{clean} \|
\end{align}

\begin{align}
    \bmx_t = \bar{\alpha}_t \bmx_0 + \sqrt{1 - \bar{\alpha}_t} \boldsymbol{\varepsilon}
\end{align}

Bayes rule:
\begin{align}
    \bmx_{t-1} =&  \frac{\sqrt{\alpha_t}(1 - \bar{\alpha}_{t-1})}{1 - \bar{\alpha}_{t}}\bmx_{t} + \frac{\sqrt{\bar{\alpha}_{t-1}}(1 - \alpha_{t})}{1 - \bar{\alpha}_{t}}\bmx_{0} \nonumber \\
    &+ \frac{(1 - \alpha_{t})(1 - \bar{\alpha}_{t-1})}{1 - \bar{\alpha}_{t}}
\boldsymbol{\varepsilon} \\
=& \frac{\bar{\alpha}_t \sqrt{\alpha_t}(1 - \bar{\alpha}_{t-1}) + \sqrt{\bar{\alpha}_{t-1}}(1 - \alpha_{t})
}{1 - \bar{\alpha}_{t}} \bmx_0
\end{align}

\begin{comment}
In general, the goal of the forward diffusion process described in Eq~\ref{eq:single_step_forward}, is to gradually introduce noise to an observation $x_0$ sampled from the a data distribution $p_0(x)$ for some set of time steps $\{1,2,..T\}$, such that $x_t$ can be reliably sampled from some noise distribution $P_T(x)$. By designing the dimension of the support of $P_T(x)$ to be the dimension of a projected $x^{\prime}$, we can mimic this transformation in the resulting space of the projection. By the result of theorem~\ref{thr:wash_out_in_projection_space}, we see that if a clean observation $x_0$ and an attacked observation $x_a$ begin in the projected subspace, we can expect similar behavior of both observations 'washing out' towards $x_t$, a behavior that was previously observed in \cite{ho2020denoising}.




\begin{theorem}
\label{thr:wash_out_in_projection_space}
Let  $\{\beta_t\in (0,1)\}^T_{t=1}$ be a variance schedule for some Markov chain that gradually adds noise (Ex: Gaussian) with support dimension $dim(x)$: \[q(x_{1:T}|x_0) = \Pi^{T}_{t=1}q(x_t|x_{t-1})\] where:

\[ q(x_{t}|x_{t-1}) := \mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1},\beta_t  I) \] Then it is expected that for some $t$ large, the adversarial's distribution $q(\Tilde{X}_t)$, and the clean distribution $q(X_t)$ will have low KL divergence: $KL[q({X}_{a_t})||q(X_t)]\leq\epsilon$, due to the eventual convergence of both  towards Gaussian noise. 
 % (Ex:
 %  $q(x^{\prime}_t|x^{\prime}_0)$ = $\mathcal{N}(x^{\prime}_t;\sqrt{\overline{\alpha}_t}x^{\prime}_{0},(1-\overline{\alpha}_t)\bold{I})$, for $\alpha_t = 1 - \beta_t$ and $\overline{\alpha}_t =\Pi^{t}_{s=1}\alpha_s$).
\end{theorem}

{\color{red} Minh's note: The original Theorem~\ref{thr:wash_out_in_projection_space} is stated for the convergence of the conditional distributions of $x_0$ and $x_a$ (for arbitrary $x$ and $x_a$) which most likely cannot be correct. The correctness of that statement would imply the output of the model would be the same for all inputs. This version of the Theorem is not stated "point-wise", i.e., it is the convergence in marginal probability.}
\Geigh{Manish TODO  -- I havent gotten to 3.3 yet, so I cant state what its current usefulness is.}

{\color{red} Minh's note: You will need Theorem~\ref{thr:wash_out_in_projection_space} to validate the next Theorem}

To see why the above result is correct, we first define constants $\alpha_t = 1 -\beta_t$ and $\Bar{\alpha}_t = \prod_{i=1}^t \alpha_i$. We then have $q(x_{t}|x_0) =  \mathcal{N} (x_t; \sqrt{\Bar{\alpha}_t} x_0, (1 -\Bar{\alpha}_t)I  )$. When $t$ is large enough, we have $\Bar{\alpha}_t$ approaches $0$, and $q(x_{t}|x_0)$ becomes close to $\mathcal{N} (x_t; 0, I  ) $. In other words, both the adversarial's distribution $q({X}_{a_t})$, and the clean distribution $q(X_t)$ converge to $\mathcal{N} (0, I  ) $ for $t$ large. Therefore, $KL[q({X}_{a_t})||q(X_t)]$ approaches $KL[\mathcal{N} (0, I  )||\mathcal{N} (0, I  )] = 0$.
\end{comment}

% Convergence follows by representing the sequential perturbation from the noise distribution as a diffusion kernel, of which can be interpreted as a Gaussian convolution if the noise distribution is selected to be a Gaussian~\cite{getreuer2013survey} \Geigh{i.e Prove that the forward process 'washes away' both adversarial and clean observations to isotopic Gaussians for sufficient T}. 

% We hypothesize that there exists a sufficient $\hat{t}$, s.t diffusing a projected observation $x_a$ that was originally attacked on the input space, for $\hat{t}$ steps yields the attacked components of the projected observation to become mainly dominated by the Gaussian perturbations, rather than purposeful adversarial perturbations.  
\subsubsection*{Reconstruction of denoised latent features}
Given that the fine-grained denoising process of a diffusion model provides a way to help filter out noise and irrelevant information, we first utilize the tensor decomposition (tucker) to project an input image $x_0$ to a low-rank latent space to more easily target the data's most significant features. We begin with collecting the factors $U2,U3,U4,U5$ from the target dataset's tucker decomposition. Once $U2,U3,U4,U5$ are collected, we project $x_0$ into the low rank space to retrieve $x^{\prime}$ via the mode multiplication of: $x^{\prime}_0 = x_0 \times_{2} U^{T}_2 \times_{3} U^T_{3} \times_{4} U^{T}_{4} \times_{5} U^{T}_{5}$. We refer to the computation of $x^{\prime}_0$ as our encoder for this model moving forward. Note that the encoder is not trained at any point. \\\\
\begin{theorem}
Given a data instance \(x_0\) projected into a lower-dimensional space using Tucker factor matrices \(U_2, U_3, U_4, U_5\) to obtain \(x^{\prime}_0 = x_0 \times_{2} U^{T}_2 \times_{3} U^T_{3} \times_{4} U^{T}_{4} \times_{5} U^{T}_{5}\), and a denoising diffusion function \( f(x) \) applied to \( x^{\prime}_0 \) yielding the denoised latent representation \( \hat{x}^{\prime}_0 = f(x^{\prime}_0) \), the reconstruction of \(\hat{x_0}\) from \(\hat{x}^{\prime}_0\) via \(\hat{x}_0 = \hat{x}^{\prime}_0 \times_{5} U_{5} \times_{4} U_{4} \times_{3} U_{3} \times_{2} U_{2}\) introduces a reconstruction error \(E_{recon}\) between the original data instance \(x_0\) and its reconstructed version \(\hat{x}_0\), defined by \(E_{recon} = ||x_0 - \hat{x}_0||\). This error can be decomposed into two components: the approximation error due to Tucker decomposition and projection \(E_{Tucker}\), and the denoising error \(E_{denoise}\) introduced by the diffusion function, such that:

\[E_{recon} \leq E_{Tucker} + E_{denoise},\]

where \(E_{Tucker}\) represents the error introduced by not capturing the full variance in each mode of \(x_0\) through the Tucker decomposition and projection process, and \(E_{denoise}\) represents the additional error introduced by the denoising diffusion process \(f(x)\).

Considering \(x_1\) as an adversarially perturbed version of \(x_0\), and applying the same denoising diffusion process to its projection \(x^{\prime}_1\), the error bound \(E_{adv}\) between the reconstructed versions of the original and adversarial instances \(\hat{x}_0\) and \(\hat{x}_1\), can be influenced by both the Tucker decomposition and the effectiveness of the denoising diffusion process in mitigating adversarial perturbations:

\[E_{adv} \leq E_{Tucker} + \Delta E_{denoise},\]

where \(\Delta E_{denoise}\) accounts for the difference in denoising effectiveness between the original and adversarially perturbed instances. The overall effectiveness of the denoising diffusion process in reducing \(E_{adv}\) is contingent upon its capacity to neutralize adversarial perturbations aligned with less significant components of the data structure diminished in the low-rank approximation.
\end{theorem}

Once the image has successfully been projected into the low rank space, the diffusion model is trained within the low-rank space. The trainable parameters are only found within the diffusion model. Finally, we project outward via the decoder, which is exactly the inverse transformation of the encoder, that is: $\hat{x}_0 = x^{'}_0 \times_{5} U_{5} \times_{4} U_{4} \times_{3} U_{3} \times_2 U_{2}$, where $\hat{x}$ is expected to have small error for all N pixels of $x_0$: $\sum^N_i || x_{0_{i}} - \hat{x}_{0_i}|| \leq \epsilon$.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/denoiser_arch_v2.drawio.png}

    \caption{Caption \cite{ho2020denoising}}
    \label{fig:enter-label}
\end{figure}

\paragraph{Usage as a purification model}
Although the model should have the potential to generate an observation from isotropic Gaussian noise, we always utilize the trained low-rank diffusion model as a purifier with $x_0$ as input. Hence, once the model is trained on low-rank space, it is necessary to choose $\hat{t}$ sufficiently well s.t adversarial perturbations are relaxed, but information retained is also sufficiently different from the noisy distribution s.t the classifier's performance is not entirely compromised~\cite{lee2023robust}. Its immediately clear that due to this trade off, we analyze the possibility of constructing a \hat{t} given the tucker projection into low-rank space.
%\Geigh{ (TODO There requires some connection to tucker reconstruction here to discuss what $\hat{t}$ should be, refer to section 4.3 for~\cite{wang2022guided}, and section 3.1 for~\cite{nie2022diffusion}. and \cite{lee2023robust}}
\begin{comment}
{\color{red} Minh: Theorem~\ref{thr:wash_out_in_projection_space} states that the distributions of the adversarial representations and the clean data's representations converge in DDPM, i.e., $KL[q({X}_{a_t})||q(X_t)]$ approaches $0$ as $t$ increases . However, to use DDPM for purification, we need to recover a clean data $x$ from its adversarial $x_a$. For that, we would need  $KL[q(x_{a_{{t}}}|x_{a_0}) || q(x_{{t}}|x_0)]$ to be small. Since the convergence in the probability does not imply point-wise convergence. We need to be more careful in choosing the time step $t$ to recover the clean data. In fact, the issue for a \textit{too-large} $t$ is that, while the distance between $x$ and $x_a$ can be small, the distance between their latent representations $x_{{t}}$ and $x_{a_{{t}}}$ can be large as $t$ increases.

Now we can see how the usage of Tucker-decomposition can help alleviate the problem. [I am not familiar with the language for the Tucker-decomposition, I will just attempt to describe my intuition here:] The assumption is that, the Tucker-decomposition is able to eliminate some portion of the adversarial noise, i.e., it reduces the \textit{raw} distance between $x$ and its adversarial counterpart $x_a$. This helps reduce the distance between their latent representations $x_{{t}}$ and $x_{a_{{t}}}$, thus, a lower $KL[q(x_{a_{{t}}}|x_{a_0}) || q(x_{{t}}|x_0)]$. [Now, we can move to the Theorem below, in which we assume  $KL[q(x_{a_{{t}}}|x_{a_0}) || q(x_{{t}}|x_0)]$ is smaller than some $\epsilon$.]}


% \Geigh{I see, this is a good catch, we may want to adjust for epsilon divergence, and suggest that we can recover at some t and denoise to clean data at t=0.}
\Geigh{I agree, so you are suggesting that beginning with the tucker decomposition allows for abstracting $x_a$ towards a likely $x_0$? But how does that solve the issue of suggesting  the existence of $\epsilon$ resulting for $t$ timesteps s.t that $X_0$ is recoverable?}
{\color{red} Minh: it increases the chance to find a feasible $t$; however, it does not pinpoint the $t$. To see this, if $|x_a - x|$ is large, there might not exist any $t$ so that we can recover $x$ from $x_a$; however, if there is a module before the DDPM to eliminate some of that difference, it makes  $|x_a(after process) - x|$ smaller, it is more likely to exist a $t$ to recover $x$.}
\Geigh{I like that angle, in that sense, you have to relax the assumption to suggest that you could recover a sample from the distribution at $t\rightarrow \infty$?, youd hope that its $x_0$, but the true $x_0$ might to difficult to recover}

{\color{red} Minh: I did not use that assumption. What Theorem 3.2 says is that you can recover the distribution $X$, not the data point $x$. In the probability sense, the Theorem 3.2 suggests it is feasible to recover "most" of the $x$ if $x_a$ is not that different from $x$. it does not say anything about all $x$}
\Geigh{It appears that 3.2 seems to suggest that the two distributions will eventually converge, but currently doesn't speak on recovering the clean distribution, the hypothesis is that if you can diffuse to some t s.t the data resembles some state that the denoiser initially trained on, then it should be likely that you can recover \textit{something} from the training distribution, but we never suggest that line of thought formally anywhere currently... and if the adversarial image has been diffused to a timestep similar what the model has seen (worst case $t\rightarrow\infty$) then we assume: That denoising from that time step improves the probability of generating the true $x_0$}
\end{comment}
\begin{theorem}
Given a data instance $x_0$ subjected to adversarial perturbation resulting in $x_a$, and its projection into a Tucker-decomposed low-dimensional space as $x^{\prime}_a = x_a \times_{2} U^{T}_2 \times_{3} U^T_{3} \times_{4} U^{T}_{4} \times_{5} U^{T}_{5}$, consider the application of a denoising diffusion process defined by a variance schedule $\{\beta_t\in (0,1)\}^T_{t=1}$ over $T$ steps, resulting in a sequence $x^{\prime}_{a_t} = f(x^{\prime}_{a_{t-1}})$, where $f(\cdot)$ denotes the denoising diffusion operation. The objective is to determine an optimal $\hat{t}$ such that for any adversarial instance $x_a$ and its clean counterpart $x_0$, the KL divergence $KL[q_a(x^{\prime}_{a_{\hat{t}}}|x^{\prime}_{a_0}) || q(x^{\prime}_{\hat{t}}|x^{\prime}_0)] \leq \epsilon$, indicating the adversarial perturbations are predominantly replaced by Gaussian noise, effectively diminishing their impact.

We hypothesize that there exists a sufficient $\hat{t}$, such that diffusing the projected observation $x^{\prime}_a$ for $\hat{t}$ steps yields the attacked components of the projection to become mainly dominated by the Gaussian perturbations introduced by the denoising diffusion, rather than the purposeful adversarial perturbations. Formally, for the denoising diffusion process characterized by the variance schedule $\{\beta_t\}$, and under the assumption that the Tucker decomposition effectively isolates significant data components while diminishing less relevant or adversarial noise:

\[ \hat{t} = \min \left\{ t \in \mathbb{N} \mid KL[q_a(x^{\prime}_{a_t}|x^{\prime}_{a_0}) || q(x^{\prime}_t|x^{\prime}_0)] \leq \epsilon, \forall t \in \{1, \ldots, T\} \right\}. \]

This $\hat{t}$ represents the minimal diffusion step at which the projection and subsequent diffusion process sufficiently "washes out" the adversarial perturbations, aligning the perturbed data closely with the distribution of the clean, diffused data in the latent space.
\end{theorem}


==> sec/4_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\paragraph{Adversarial Purification} The use of generative models has become a widely practiced approach towards defending against adversarial attacks~\cite{DBLP:journals/corr/abs-1805-06605}~\cite{DBLP:journals/corr/abs-2106-06041}, with diffusion based defenses seeming to be the best defense against white box attacks. Recently, techniques aimed to improve diffusion based purification techniques are beginning to receive much attention~\cite{kang2024diffattack}~\cite{yuezhang2024dissecting}~\cite{287372}. For this work we also consider the vanilla implementations~\cite{nie2022DiffPure}~\cite{wang2022guided}, as a baseline and highlight the use cases in which our methods are beneficial towards performance.
